A vision foundation model for single-cell biology via spatial gene cartography

Most single-cell foundation models are adapted from language models, representing each cell as a sequence of gene tokens. This discards the relationships among genes and often the magnitude of their expression. We present scVision, a vision foundation model that instead renders each cell as a continuous image. Using optimal transport, it places genes at fixed positions on a single shared, pan-tissue layout so that co-expressed genes become spatial neighbours, turning a transcriptome into an image in which gene programs appear as local texture. We pretrain a vision transformer by masked image modelling on 72 million human cells and use the frozen encoder with no fine-tuning. In zero-shot evaluations on six independent, held-out studies, scVision is the most accurate cell-type annotator and recovers gene programs without supervision, ahead of existing foundation models and classical baselines; on multi-study integration it matches the strongest token-based model while conserving the most biological structure, without ever seeing a batch label. Permuting the gene layout with the network fixed sharply lowers accuracy, more than removing the vision transformer itself, showing that biologically meaningful position, not the network, carries the signal. By preserving expression magnitude and gene relationships, scVision reframes single-cell representation learning as a vision problem, connecting it to the mature methods of computer vision.

==> latexmkrc <==
# latexmkrc -- build the standalone Supplementary Information BEFORE the main
# article so that the cross-document references resolve.
#
# Why this file exists
# --------------------
# The Supplementary Information is a SEPARATE standalone document
# (supplement.tex, auto-generated by figures/make_supplement.py). The main
# article (main.tex) pulls the supplement's S-numbered figure/table numbers via
#
#     \usepackage{xr}
#     \externaldocument{supplement}
#
# xr substitutes those numbers by reading supplement.aux. If supplement.aux does
# not exist at the moment main.tex is compiled, the references print as "??"
# (e.g. "Supplementary Fig. ??", "Supplementary Table ??").
#
# This file makes latexmk compile supplement.tex first (creating supplement.aux)
# whenever it builds the main article, so the references always resolve. It
# works locally (`latexmk main.tex`) and on Overleaf, which drives compilation
# with latexmk and reads this file automatically. Once supplement.aux exists,
# latexmk's normal multi-pass build of main.tex substitutes the real S-numbers.
#
# Engine note: if your Overleaf project's compiler is XeLaTeX or LuaLaTeX rather
# than pdfLaTeX, change the "-pdf" in the system() call below to "-xelatex" or
# "-lualatex". (For xr only the .aux labels matter, and those are identical
# across engines, so pdfLaTeX here is fine even if the article uses another
# engine.)

{
    # Guards that decide whether to pre-build the supplement:
    #   $nested   recursion guard. The nested `latexmk ... supplement.tex` call
    #             re-reads this same file; the environment variable (inherited
    #             through system()) tells that inner run NOT to pre-build again.
    #   $is_supp  a direct `latexmk supplement.tex` is already building the
    #             supplement, so no pre-build is needed.
    #   $is_clean do not compile anything during a latexmk cleanup (-c/-C/-gg).
    my $nested   = $ENV{__SCV_SUPP_PREBUILD__};
    my $is_supp  = grep { /supplement/  } @ARGV;
    my $is_clean = grep { /^-(c|C|gg)$/ } @ARGV;

    unless ( $nested || $is_supp || $is_clean ) {
        $ENV{__SCV_SUPP_PREBUILD__} = 1;   # inherited by the nested latexmk
        warn "latexmkrc: pre-building supplement.tex so xr cross-references resolve...\n";
        system( 'latexmk', '-pdf', '-interaction=nonstopmode', 'supplement.tex' );
    }
}

